Transient Finite Element Simulation of Accelerator Magnets Using Thermal Thin Shell Approximation

Thermal transient responses of superconducting magnets can be simulated using the finite element (FE) method. Some accelerator magnets use cables whose electric insulation is significantly thinner than the bare electric conductor. The FE discretisation of such geometries with high-quality meshes leads to many degrees of freedom. This increases the computational time, particularly since non-linear material properties are involved. In this work, we propose to use a thermal thin-shell approximation (TSA) to improve the computational efficiency when solving the heat diffusion equation in two dimensions. We apply the method to compute the thermal transient response of superconducting accelerator magnets used for CERN's Large Hadron Collider (LHC) and High-Luminosity LHC. The TSA collapses thin electrical insulation layers into lines while accurately representing the thermal gradient across the insulation's thickness. The TSA is implemented in the multipole module of the open-source Finite Element Quench Simulator (FiQuS), which can generate the multipole magnet models programmatically from input text files. First, the TSA approach is verified by comparison to classical FE simulations with meshed surface insulation regions for a simple block of four cables and a detailed model of the MBH dipole. The results show that the TSA approach reduces the computational time significantly while preserving the accuracy of the solution. Second, the quench heater (QH) delay computed with the TSA method is compared to measurements for the MBH magnet. To this end, the thermal transient simulation is coupled to a magnetostatic solution to account for magneto-resistive effects. Third, the TSA's full capabilities are showcased in non-linear magneto-thermal simulations of several LHC and HL-LHC superconducting magnet models. The full source code, including all input files, is publicly available.

==> figures/features_and_capabilities/yaml_showcase.tex <==
\begin{yaml_box}
\lstinputlisting{figures/features_and_capabilities/yaml_showcase.yaml}
\end{yaml_box}

==> figures/features_and_capabilities/yaml_showcase_4_conductors.tex <==
\begin{yaml_box}
\lstinputlisting{figures/features_and_capabilities/yaml_showcase_4_conductors.yaml}
\end{yaml_box}

==> figures/features_and_capabilities/yaml_showcase_qh.tex <==
\begin{yaml_box}
\lstinputlisting{figures/features_and_capabilities/yaml_showcase_qh.yaml}
\end{yaml_box}

==> figures/tikz_plots_4cond/rel_error_over_time.tex <==
\pgfplotstableread[col sep=comma,]{data_4cond/time_steps.csv}\timeSteps
\pgfplotstableread[col sep=comma,]{data_4cond/rel_error_time_ref.csv}\ErrRef
\pgfplotstableread[col sep=comma,]{data_4cond/rel_error_time_tsa.csv}\Errtsa

\pgfplotstablecreatecol[copy column from table={\timeSteps}{0}]{timeSteps}{\ErrRef}
\pgfplotstablecreatecol[copy column from table={\timeSteps}{0}]{timeSteps}{\Errtsa}

\begin{tikzpicture}

    \begin{axis}[cycle list={[
        colormap/viridis, 
        colors of colormap={0, 300, 0, 300}]},
        width=.47\textwidth,
        height=5cm,
        xlabel={Time (\si{\milli \second})},
        ylabel={Rel error (\%)}, 
        ylabel near ticks, 
        legend columns=2, 
        legend style={font=\footnotesize, at={(0.01, 0.99)}, anchor=north west}, 
        ticklabel style = {font=\scriptsize},
        legend style={font=\scriptsize},
        label style={font=\small},
        legend image post style={mark indices={}}, 
        ytick scale label code/.code={}, 
        legend cell align={left},
        legend image post style={mark indices={}}, 
        ymode=log,
        x filter/.code={\pgfmathparse{#1*1000}\pgfmathresult}
         ]

      \addplot+[
                mark=none,
                thick
            ] 
         table[
            x = timeSteps,
            y index = 4
        ] 
        {\ErrRef};%

    \addplot+[
                mark=none,
                thick
            ] 
         table[
            x = timeSteps,
            y index = 0
        ] 
        {\ErrRef};%

    \addplot+[
    mark=none,
    mymark={o}{solid, opacity=1}, 
    opacity=0,
    thick
        ] 
     table[
        x = timeSteps,
        y index = 4
    ] 
    {\Errtsa};%

    \addplot+[
    mark=none,
    mymark={o}{solid, opacity=1}, 
    opacity=0,
    thick
    ] 
     table[
        x = timeSteps,
        y index = 0
    ] 
    {\Errtsa};%

         
    \legend{sur msh 1, sur msh 2, TSA msh 1, TSA msh 2}
    
    \end{axis}%
\end{tikzpicture}
